Equivariant and Invariant Reynolds Networks

Invariant and equivariant networks are useful in learning data with symmetry, including images, sets, point clouds, and graphs. In this paper, we consider invariant and equivariant networks for symmetries of finite groups. Invariant and equivariant networks have been constructed by various researchers using Reynolds operators. However, Reynolds operators are computationally expensive when the order of the group is large because they use the sum over the whole group, which poses an implementation difficulty. To overcome this difficulty, we consider representing the Reynolds operator as a sum over a subset instead of a sum over the whole group. We call such a subset a Reynolds design, and an operator defined by a sum over a Reynolds design a reductive Reynolds operator. For example, in the case of a graph with $n$ nodes, the computational complexity of the reductive Reynolds operator is reduced to $O(n^2)$, while the computational complexity of the Reynolds operator is $O(n!)$. We construct learning models based on the reductive Reynolds operator called equivariant and invariant Reynolds networks (ReyNets) and prove that they have universal approximation property. Reynolds designs for equivariant ReyNets are derived from combinatorial observations with Young diagrams, while Reynolds designs for invariant ReyNets are derived from invariants called Reynolds dimensions defined on the set of invariant polynomials. Numerical experiments show that the performance of our models is comparable to state-of-the-art methods.

==> exp.tex <==
We evaluated our models compared to fully-connected neural nets (FNNs) and \citet{maron2018invariant} using synthetic datasets for equivariant and invariant tasks.
%
In the experiments, we used two models; Reynolds Networks (ReyNets) and $4$-reduced Reynolds Networks (4red-ReyNets).


\subsection{Datasets}
We created four types of synthetic datasets for the comparison.
Given an input matrics data $\mathbf{A} \in \mathbb{R}^{n \times n}$, each task is defined by:
\begin{itemize}
    \item \textbf{Symmetry}: projection onto the symmetric matrices $F(\mathbf{A})=\frac{1}{2}(\mathbf{A} + \mathbf{A}^\top)$,
    \item \textbf{Diagonal}: diagonal extraction $F(\mathbf{A})=diag(\mathbf{A})$,
    \item \textbf{Power}: computing each squared element $F(\mathbf{A})=[A_{i,j}^2]$,
    \item \textbf{Trace}: computing the trace $F(\mathbf{A})=tr(\mathbf{A})$,
\end{itemize}
where the task function $F$ is equivariant in \textit{symmetry}, \textit{diagonal}, and \textit{power}, and is invariant in \textit{trace}.
Following \citet{maron2018invariant}, we sampled i.i.d. random matrices $\mathbf{A}$ with uniform distribution in $[0, 10]$; then we transformed it by the task function $F$.
In our experiments, we provided $n \in \{ 3, 5, 10, 20\}$, and the size of training dataset and test dataset is 1000 respectively. 


\subsection{Implementation Details}
For equivariant tasks, we applied equivariant ReyNets.
For invariant tasks, we applied invariant ReyNets following the architecture of the invariant model proposed by \citet{maron2018invariant};
an equivariant ReyNet is followed by max pooling\footnote{This operation outputs the max value of diagonal and non-diagonal elements of an input matrix.}, and fully-connected layers.
We adopted the ReLU function as activation.
We used Adam optimizer and set learning rate as 1e-3 and weight decay as 1e-5.
Batch size is 100.
Note that the models of \citet{maron2018invariant} are re-implemented by PyTorch in reference to the author's implementation in Tensorflow. 

In terms of an objective function, we modified mean squared error (MSE) loss based on Theorem \ref{represention}.
In a straightforward manner, equivariant tasks are regression task so that MSE loss is selected to decrease the gap of all elements between an output matrix and ground truth matrix: $\ell_{std}\colon \mathbb{R}^{n\times n} \times \mathbb{R}^{n\times n} \rightarrow \mathbb{R}$.
However, thanks to Theorem \ref{represention}, ReyNet does not require calculating whole elements but the gap of 1st row of 1st column element and 1st row of 2nd column element: $\ell_{corner}\colon \mathbb{R}^{1\times 2} \times \mathbb{R}^{1\times 2} \rightarrow \mathbb{R}$.
In this paper, we call the latter objective function as corner MSE loss.

\subsection{Results}
\begin{wraptable}[10]{r}[0mm]{50mm}
 \caption{Comparison of Objective Function}
 \label{tab:exp2}
 \centering
 \small
    \begin{tabular}{l|ll}
    \toprule
        $n$    & mse & corner mse \\ \midrule
        3 & 1.438e-4 & \textbf{1.249e-4} \\
        5 & \textbf{4.912e-5} & 9.375e-5 \\
        10 & 1.157e-4 & \textbf{6.487e-5} \\
        20 & 1.608e-4 & \textbf{8.537e-5} \\ \bottomrule
    \end{tabular}
\end{wraptable}
Table \ref{tab:exp1} shows the result of synthetic datasets, which is the average of MSE of five different seeds.
As a result, our proposed models outperform \citet{maron2018invariant} overall.
% Especially, with regards to \textit{symmetry} and \textit{diagonal} tasks, both orders of magnitude were better than \citet{maron2018invariant}.
Interestingly, with regards to the \textit{power} task, FNN and ReyNet are worse than other models.
The function $F$ of \textit{power} task amplifies the output error to large value.
Simultaneously, when the number of parameters of the model is very large along with the size of $n$, the output of the model becomes sensitive.
Therefore, we considered that the error became large due to the combination with large neural networks and the \textit{power} function.
% In other hand, \citet{maron2018invariant} and ReyNet is designed independent to size $n$ 


Moreover, we validated the effect of an objective function.
We trained 4r-ReyNets with standard MSE loss and Corner MSE loss respectively.
Table \ref{tab:exp2} shows the result of using each objective function.
Accordingly, Corner MSE loss achieved lower error than standard MSE loss except for $n=5$ case.
Therefore, using Corner MSE loss is a good choice for equivariant tasks.
%\begin{table}[t]
%    \centering
%    \caption{Comparison of Objective Function}
%    \begin{tabular}{l|ll}
%    \toprule
%            & MSE & Corner MSE \\ \midrule
%        n=3 & 1.438e-4 & \textbf{1.249e-4} \\
%        n=5 & \textbf{4.912e-5} & 9.375e-5 \\
%        n=10 & 1.157e-4 & \textbf{6.487e-5} \\
%        n=20 & 1.608e-4 & \textbf{8.537e-5} \\ \bottomrule
%    \end{tabular}
%    \label{tab:exp2}
%\end{table}

\subsection{Generalization Error}
\begin{figure}[t]
    \centering
  \begin{minipage}[b]{0.45\hsize}
    \centering
    \includegraphics[width=0.95\columnwidth]{iclr2022/figs/symmetry-compare.pdf}
    \subcaption{Symmetry}\label{gen-sym}
  \end{minipage}
  \begin{minipage}[b]{0.45\hsize}
    \centering
    \includegraphics[width=0.95\columnwidth]{iclr2022/figs/power-compare.pdf}
    \subcaption{Power}\label{gen-diag}
  \end{minipage}
  \caption{Generalization Error}\label{fig:generalization}
\end{figure}
Notably, our 4red-ReyNet does not depend on the size of inputs $n$.
In order to test the generalization performance, we trained 4red-ReyNet with $n_{train}=3$ dataset and then validated the MSE on $n_{test}\in \{3, 4, \dots, 20\}$ datasets. 
The results are depicted in Figure \ref{fig:generalization}.
We can see that our 4-reduced ReyNet is generalized to the input size.
Note that with regard to invariant tasks, we confirmed the model is not generalized to the tasks as \citet{maron2018invariant} has reported.
% This might be because the fully-connected layer following a ReyNet cannot be generalized.


==> table-1.tex <==
% % Please add the following required packages to your document preamble:
% % \usepackage{booktabs}
% \begin{table}[]
% \caption{Results of comparison to baseline methods}
% \footnotesize
% \begin{tabular}{@{}lllllllllllllllllllll@{}}
% \toprule
% Task                & \multicolumn{4}{l}{Symmetry}                                                  & \multicolumn{4}{l}{Diagonal}                                                  & \multicolumn{4}{l}{Power}                                                     & \multicolumn{4}{l}{Trace}                                                     & \multicolumn{4}{l}{Non-Diagonal Sum}                                       \\
% \textit{\textbf{n}} & 3                 & 5                 & 10                & 20                & 3                 & 5                 & 10                & 20                & 3                 & 5                 & 10                & 20                & 3                 & 5                 & 10                & 20                & 3                 & 5                 & 10                & 20             \\ \midrule
% \citet{maron2018invariant}               & 6.600e-3          & 3.786e-3          & 9.294e-4          & 4.471e-3          & 2.065e-3          & 2.266e-3          & 4.098e-3          & 4.743e-4          & 4.036e-1          & 3.462e-1          & 7.062e-1          & 4.735e-1          & 1.241e-3          & 6.696e-3          & 3.663e-2          & 5.527e-2          & 5.092e-2          & 5.333e-2          & 8.197e-1          & 6.975          \\
% ReyNet (ours)     & 2.147e-4          & 3.960e-4          & 1.408e-3          & 3.151e-3          & 1.007e-4          & 2.472e-4          & 6.635e-4          & 1.112e-4          & 3.798e-1          & 1.257             & 3.620             & 3.065             & 1.884e-3          & 2.949e-3          & 4.275e-2          & 5.338e-2          & \textbf{3.452e-3} & \textbf{1.869e-2} & \textbf{2.056e-1} & \textbf{1.472} \\
% 4r-ReyNet (ours)         & \textbf{8.544e-5} & \textbf{4.889e-5} & \textbf{7.529e-5} & \textbf{6.554e-5} & \textbf{6.947e-5} & \textbf{1.932e-5} & \textbf{5.568e-5} & \textbf{3.566e-5} & \textbf{1.204e-1} & \textbf{1.330e-1} & \textbf{1.217e-1} & \textbf{1.165e-1} & \textbf{3.491e-4} & \textbf{1.914e-3} & \textbf{6.758e-3} & \textbf{1.220e-2} & 1.352             & 4.428e+1          & 3.763e+2          & 2.146e+3       \\ \bottomrule
% \end{tabular}
% \end{table}
% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
% \begin{table}[]
% \centering
% \caption{Results of comparison to a baseline method}
% \fontsize{8pt}{9pt}\selectfont
% % \footnotesize
% \begin{tabular}{@{}lllllllll@{}}
% \toprule
% Task                & \multicolumn{4}{l}{Symmetry}                                                  & \multicolumn{4}{l}{Diagonal}                                                  \\
% \textit{\textbf{n}} & 3                 & 5                 & 10                & 20                & 3                 & 5                 & 10                & 20                \\ \midrule
% \citet{maron2018invariant}               & 6.600e-3          & 3.786e-3          & 9.294e-4          & 4.471e-3          & 2.065e-3          & 2.266e-3          & 4.098e-3          & 4.743e-4          \\
% ReyNet (ours)     & 2.147e-4          & 3.960e-4          & 1.408e-3          & 3.151e-3          & 1.007e-4          & 2.472e-4          & 6.635e-4          & 1.112e-4          \\    
% 4r-ReyNet (ours)         & \textbf{8.544e-5} & \textbf{4.889e-5} & \textbf{7.529e-5} & \textbf{6.554e-5} & \textbf{6.947e-5} & \textbf{1.932e-5} & \textbf{5.568e-5} & \textbf{3.566e-5} \\ \bottomrule
% \toprule
% Task                & \multicolumn{4}{l}{Power}                                                     & \multicolumn{4}{l}{Trace}                                                     \\
% \textit{\textbf{n}} & 3                 & 5                 & 10                & 20                & 3                 & 5                 & 10                & 20                \\ \midrule
% \citet{maron2018invariant}               & 4.036e-1          & 3.462e-1          & 7.062e-1          & 4.735e-1          & 1.241e-3          & 6.696e-3          & 3.663e-2          & 5.527e-2          \\
% ReyNet (ours)     & 3.798e-1          & 1.257             & 3.620             & 3.065             & 1.884e-3          & 2.949e-3          & 4.275e-2          & 5.338e-2          \\
% 4r-ReyNet (ours)         & \textbf{1.204e-1} & \textbf{1.330e-1} & \textbf{1.217e-1} & \textbf{1.165e-1} & \textbf{3.491e-4} & \textbf{1.914e-3} & \textbf{6.758e-3} & \textbf{1.220e-2} \\ \bottomrule
% \end{tabular}
% \label{tab:exp1}
% \end{table}

\begin{table}[]
\centering
\caption{Results of comparison to a baseline method}
\fontsize{8pt}{9pt}\selectfont
% \footnotesize
\begin{tabular}{@{}lllllllll@{}}
\toprule
Task                & \multicolumn{4}{l}{Symmetry}                                                  & \multicolumn{4}{l}{Diagonal}                                                  \\
\textit{\textbf{n}} & 3                 & 5                 & 10                & 20                & 3                 & 5                 & 10                & 20                \\ \midrule
FNN               & 1.730e-4          & 9.180e-4          & 1.454e-3          & 3.0583          & 1.295e-4          & 2.655e-4          & 1.148e-4          & 1.081e-1          \\
\citet{maron2018invariant}               & 6.600e-3          & 3.786e-3          & 9.294e-4          & 4.471e-3          & 2.065e-3          & 2.266e-3          & 4.098e-3          & 4.743e-4          \\
ReyNet (ours)     & 2.147e-4          & 3.960e-4          & 1.408e-3          & 3.151e-3          & 1.007e-4          & 2.472e-4          & 6.635e-4          & 1.112e-4          \\    
4red-ReyNet (ours)         & \textbf{8.544e-5} & \textbf{4.889e-5} & \textbf{7.529e-5} & \textbf{6.554e-5} & \textbf{6.947e-5} & \textbf{1.932e-5} & \textbf{5.568e-5} & \textbf{3.566e-5} \\ \bottomrule
\toprule
Task                & \multicolumn{4}{l}{Power}                                                     & \multicolumn{4}{l}{Trace}                                                     \\
\textit{\textbf{n}} & 3                 & 5                 & 10                & 20                & 3                 & 5                 & 10                & 20                \\ \midrule
FNN               & 2.586          & 3.091e+1          &    5.756e+1       & 6.268e+2          & 2.821e-4          & 1.135e-3          & 9.529e-3          & 5.149e-2          \\
\citet{maron2018invariant}               & 4.036e-1          & 3.462e-1          & 7.062e-1          & 4.735e-1          & 1.241e-3          & 6.696e-3          & 3.663e-2          & 5.527e-2          \\
ReyNet (ours)     & 3.798e-1          & 1.257             & 3.620             & 3.065             & 1.884e-3          & 2.949e-3          & 4.275e-2          & 5.338e-2          \\
4red-ReyNet (ours)         & \textbf{1.204e-1} & \textbf{1.330e-1} & \textbf{1.217e-1} & \textbf{1.165e-1} & \textbf{3.491e-4} & \textbf{1.914e-3} & \textbf{6.758e-3} & \textbf{1.220e-2} \\ \bottomrule
\end{tabular}
\label{tab:exp1}
\end{table}
